Demo Abstract: CDMA-based IoT Services with Shared Band Operation of LTE in 5G

With the vision of deployment of massive Internet-of-Things (IoTs) in 5G network, existing 4G network and protocols are inefficient to handle sporadic IoT traffic with requirements of low-latency, low control overhead and low power. To suffice these requirements, we propose a design of a PHY/MAC layer using Software Defined Radios (SDRs) that is backward compatible with existing OFDM based LTE protocols and supports CDMA based transmissions for low power IoT devices as well. This demo shows our implemented system based on that design and the viability of the proposal under different network scenarios.

==> eval.tex <==
\section{Evaluation Scenarios}
\label{sec:eval}

\eat{
\begin{figure}[t]
\begin{center}
\vspace{0.2in} \hspace{0.35in}
\epsfig{figure= pics/IoTsingleLink_setup.pdf,width=3.3in}
\end{center}
\caption{Setup of a single IoT link for uplink transmission using CDMA software implementation and USRP}
\label{fig:IoTsingleLink_setup}
\vspace{-0.6cm}
\end{figure}
\subsection{Single CDMA-based IoT Link}
\label{subsec:single}
With the test case of a single IoT UE connected to the eNB as shown in Fig~\ref{fig:IoTsingleLink_setup}, we evaluate the overall implementation robustness and characterize packet-error and packet-detect rates of IoT link with respect to the SINR. The performance is evaluated under variable IoT payload (1-15 Bytes) and inter-packet transmission delay. The scenario is also implemented and evaluated with MATLAB simulations.
}

\subsection{Data Transmission from Multiple IoT UEs}
The scenario of multiple IoT UEs connected to the single eNB poses the challenge of increased signal processing complexity at the receiver (eNB) where each UE spreads the message with separate Hadamard code and data transmission is asynchronous. Taking an example of two IoT links, as shown in Fig.~\ref{fig:IoT_eNB_twoUEs}, we evaluate the overall implementation robustness and characterize packet-error and packet-detect rates of IoT link with respect to the SINR. The performance is evaluated under variable IoT payload (1-15 Bytes) and inter-packet transmission delay {\color{blue} (need to add values). The scenario is also implemented and evaluated with MATLAB simulations.} This scenario could further be extended for multiple IoT links ($>$ 2).
\eat{
The scenario of two IoT UEs connected to the single eNB poses the challenge of increased signal processing complexity at the receiver (eNB) where each UE spreads the message with separate Hadamard code and data transmission is asynchronous. This scenario is evaluated against the metrics used in the earlier scenario. This case could further be extended for multiple ($>$ 2) UEs. 
}

\subsection{Coexistence of IoT link and LTE}
This scenario, as shown in Fig.~\ref{fig:IoT_LTE_coex}, aims to evaluate performance of the shared band operation of LTE and CDMA-underlay IoT link. In addition, this scenario gives insights on design details of CDMA-underlay IoT protocol considering OFDMA structure of LTE. As a next step, we envision the integration of IoT eNB and OAI/LTE eNB into a single eNB which processes IoT and LTE uplink traffic and schedules/send both downlink traffic.

\begin{figure}[t]
\begin{center}
\vspace{0.2in} \hspace{0.35in}
\epsfig{figure= pics/IoT_eNB_twoUEs.pdf,width=3.3in}
\end{center}
\caption{Setup of a single IoT link for uplink transmission using CDMA software implementation and USRP}
\label{fig:IoT_eNB_twoUEs}
\vspace{-0.6cm}
\end{figure}

\begin{figure}[t]
\begin{center}
\vspace{0.2in} \hspace{0.35in}
\epsfig{figure= pics/IoT_LTE_coex.pdf,width=3.3in}
\end{center}
\caption{Setup of a single IoT link for uplink transmission using CDMA software implementation and USRP}
\label{fig:IoT_LTE_coex}
\vspace{-0.6cm}
\end{figure}

